Enhancing In-Context Learning with Answer Feedback for Multi-Span Question Answering

Whereas the recent emergence of large language models (LLMs) like ChatGPT has exhibited impressive general performance, it still has a large gap with fully-supervised models on specific tasks such as multi-span question answering. Previous researches found that in-context learning is an effective approach to exploiting LLM, by using a few task-related labeled data as demonstration examples to construct a few-shot prompt for answering new questions. A popular implementation is to concatenate a few questions and their correct answers through simple templates, informing LLM of the desired output. In this paper, we propose a novel way of employing labeled data such that it also informs LLM of some undesired output, by extending demonstration examples with feedback about answers predicted by an off-the-shelf model, e.g., correct, incorrect, or incomplete. Experiments on three multi-span question answering datasets as well as a keyphrase extraction dataset show that our new prompting strategy consistently improves LLM's in-context learning performance.

==> tables/main-results-bak.tex <==
\begin{table}
\centering
\caption{Main results on MRC. The best results are bold. Add MORE INFORMATION}
\label{table:main_results1}

% \resizebox{\textwidth}{!}{
\begin{tabular}{lcc|cc|cc}

\Xhline{3\arrayrulewidth}
\multirow{2}{*}{} & \multicolumn{2}{c|}{MultiSpanQA} & \multicolumn{2}{c|}{QUOREF} & \multicolumn{2}{c}{DROP} \\
\cline{2-7}
& EM$^+$ & PM & EM & F1 & EM & F1\\
\Xhline{2\arrayrulewidth}

PLM-Based Methods &&&&&&\\
\quad BART$_\text{BASE}$ & 63.23 & 78.77 & 66.40 & 72.52 & 53.00 & 56.16
\\
\quad T5$_\text{BASE}$
& 70.83 & 84.23 & 75.00 & 79.93 & 58.20 & 60.92
\\
\quad TASE(drop,quoref robera, msqa bert)
& 54.99 & 72.59 & 79.40 & 84.8& 80.50 & 87.80
\\
\Xhline{2\arrayrulewidth}
GPT-Based Methods &&&&&&\\
\quad ChatGPT(3-shot) &&&&& - & 64.10
\\
\quad Random & 58.62 & 80.62 & 71.40 & 80.25 & 47.70 & 60.53
\\
\quad KNN$_\text{BM25}$ & 61.33 & 81.63 & 70.80 & 79.00 & 58.40 & 65.93
\\
\quad KNN$_\text{Dense}$ & 60.78 & 81.51 & 73.00 & 79.76 & 50.90 & 60.69
\\
\Xhline{2\arrayrulewidth}
Our Method & 64.60 & 83.11 & 73.60 & 80.55 & 62.00 & 69.11
\\

\Xhline{3\arrayrulewidth}
\end{tabular}

% }


\end{table}







\begin{table}
\centering
\caption{Main results on keyphrase extraction. For each dataset we report present keyphrase prediction and absent keyphrase prediction. The best results are bold. Specifically, \textsuperscript{\textbf{\textdoublebarpipe}} indicates the results in \cite{kpsurvey} and we report the results collected by \cite{GPT_Keyphrase}.}
\label{table:main_results2}
% \resizebox{\linewidth}{!}{

\begin{tabular}{lcc|cc|cc|cc}
\Xhline{3\arrayrulewidth}

\multirow{2}{*}{} & \multicolumn{4}{c|}{INSPEC} & \multicolumn{4}{c}{KRAPIVIN}\\
\cline{2-9}
\multirow{2}{*}{} & \multicolumn{2}{c|}{Present} & \multicolumn{2}{c|}{Absent} & \multicolumn{2}{c|}{Present}& \multicolumn{2}{c}{Absent}\\
\cline{2-9}
& F1@5 & F1@M & F1@5 & F1@M & F1@5 & F1@M & F1@5 & F1@M\\
\Xhline{2\arrayrulewidth}

PLM-Based Methods & & & & & &\\
\quad SciBART$_\text{BASE}$\textsuperscript{\textbf{\textdoublebarpipe}}
& 0.275 & 0.328 & 0.016 & 0.028 & 0.282 & 0.329 & 0.033 & 0.054
\\
\quad BART$_\text{BASE}$\textsuperscript{\textbf{\textdoublebarpipe}}
& 0.270 & 0.323 & 0.010 & 0.017 & 0.270 & 0.336 & 0.028 & 0.049
\\
\quad T5$_\text{BASE}$\textsuperscript{\textbf{\textdoublebarpipe}}
& 0.288 & 0.339 & 0.011 & 0.020 & 0.302 & 0.350 & 0.023 & 0.043
\\

\Xhline{2\arrayrulewidth}
GPT-Based Methods &&&&&&\\
\quad ChatGPT(zero-shot) & 0.298 & 0.417 & 0.016 & 0.030 & 0.239 & 0.187 & 0.003 
& 0.004
\\
\quad Random & 0.401 & 0.472 & 0.033 & 0.051& &
\\
\quad KNN$_\text{BM25}$ & 0.405 & 0.470 & 0.029 & 0.051 & 0.240 & 0.298 & 0.020 & 0.033
\\
\quad KNN$_\text{Dense}$ & 0.399 & 0.468 & 0.026 & 0.038 & 0.259 & 0.309 & 0.019 & 0.030
\\
\Xhline{2\arrayrulewidth}
Our Method & \textbf{0.425} & \textbf{0.499} & \textbf{0.034} & \textbf{0.055} & 0.254 & 0.294 & 0.021 & 0.035
\\

\Xhline{3\arrayrulewidth}

\end{tabular}
% }


\end{table}
